Design-Specific Transformations in Visualization

In visualization, the process of transforming raw data into visually comprehensible representations is pivotal. While existing models like the Information Visualization Reference Model describe the data-to-visual mapping process, they often overlook a crucial intermediary step: design-specific transformations. This process, occurring after data transformation but before visual-data mapping, further derives data, such as groupings, layout, and statistics, that are essential to properly render the visualization. In this paper, we advocate for a deeper exploration of design-specific transformations, highlighting their importance in understanding visualization properties, particularly in relation to user tasks. We incorporate design-specific transformations into the Information Visualization Reference Model and propose a new formalism that encompasses the user task as a function over data. The resulting formalism offers three key benefits over existing visualization models: (1) describing task as compositions of functions, (2) enabling analysis of data transformations for visual-data mapping, and (3) empowering reasoning about visualization correctness and effectiveness. We further discuss the potential implications of this model on visualization theory and visualization experiment design.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> content/intro.tex <==
The Information Visualization Reference Model  (Infovis Reference Model) by Card et al.~\cite{card1999readings} is a foundational framework in the visualization community towards understanding the mapping of data to visual elements.   The model (\Cref{fig:computemodel}(top)), semantically delineates the primary phases of visualization: Data Transformation cleans, reshapes, and summarizes the source dataset into data tables (for example to derive the desired information into a spreadsheet from a large database), Visual Mapping constructs and places marks onto the spatial substrate (for example to choose between a bar chart or a pie chart), and View Transformation provides mechanisms to change the properties of visual marks and/or manipulate the viewport. 

Organizing the steps semantically has led to clean abstractions that inform how modern visualizations are developed and evaluated.   Consider the process to visualize a pie chart. Libraries such as VegaLite, Plotly, and Matplotlib ask developers to define the data transformations used to derive the table, and simply specify the visual mapping (see Figure~\ref{fig:teaser})---the library is then responsible for computing the group statistics, percentages, and mark placements needed to construct and render the marks.  
The model also helps researchers design graphical perception experiments that isolate the effects of visualization designs by focusing on the visual mapping step in isolation of data and view transformations (see a survey by Quadri and Rosen \cite{quadri2021survey}).

Despite these broad ranging benefits, we observe that this semantic delineation obscures the process of visual mapping in a way that makes it difficult to reason about visualizations and their relationships to user tasks.   
%
Consider the four basic charts in \Cref{fig:teaser} that render a table with two numeric columns, $D(a,b)$, and how their visual mappings are specified in Vega-lite~\cite{satyanarayan2016vega}.  
From the specification, it would appear that scatterplot is most similar to the pie chart, as they only differ in the mark type and the visual attributes that \texttt{a} and \texttt{b} are mapped to, and the bar chart is most similar to the proportional stacked chart, as they only differ in that \texttt{a} is mapped to \texttt{x} instead of \texttt{color}.
Yet these syntactic similarities are superficial and contrary to our understanding of the visualization process.  For instance, that the pie chart and proportional stacked chart both encode the same information, and only differ in their encoding in a circular or a rectangular layout, respectively.


We observe that the core reason for this dissonance between visualization specifications and functions is that the Visual Mapping step represents two distinct substeps.  The first involves additional transformations over the data tables in order to compute, e.g., desired statistics and spatially place marks  that are specific to the visualization design.   We term these \textbf{Design-specific Transformations}.   The second is the visual encoding that maps each row in the transformed table to a mark, and data attributes to mark attributes using simple scaling functions.   


Simply separating design-specific transformations and visual encodings leads to immediate insights about relationships between the four charts.  For instance, the scatterplot does not apply any additional transformations and directly encodes \texttt{a}, \texttt{b} to mark attributes. In contrast, the pie chart requires a complex sequence of design-specific transformations---it groups by \texttt{a} to derive per-group sums, computes the total sum and uses it to derive per-group percentages, and then stacks the percentage values---beforing encoding the {\it derived} attributes \texttt{c}, \texttt{d}, and \texttt{perc} to mark attributes.  We can see that the stacked bar and pie chart are nearly identical and only slightly differ in their visual encodings; both are related to the bar chart, which also computes per-group sum of \texttt{a}, but nothing further.   

This separation also sheds light on the applicability of each chart to different user tasks.  For instance, pie charts are historically a controversial chart type~\cite{tufte2001visual,few2007save,pie1,pie2,siirtola2019cost} with proponents on both sides.   Its visual encoding maps the derived \texttt{perc} and \texttt{d} (stacked \texttt{perc}) attributes.   Consistent with perception studies, we would expect the pie chart to excel at percentage estimation tasks as compared to the scatterplot and bar chart, but that it is impossible to answer questions about individual input values because they have been aggregated.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/computemodel2.pdf}
    \caption{The proposed model in this paper differs from the Infovis Reference Model in two important ways: we decompose visual mappings into design-specific transformations (e.g., stacking, quantization, calculating statistics) from visual encoding, and we model the task $q(D)$ as a function over the input dataset that the user wishes to estimate.}
    \label{fig:computemodel}
\end{figure}

Based the above observations, this paper proposes a {\it Transform-centric Model} (\Cref{fig:computemodel}(bottom)) that extends the Infovis Reference Model in two small but important ways.  First, it expands visual mappings to explicitly model design-specific transformations and visual encoding, so that the visual abstraction $V$ is the output of applying design-specific transformations and visual encoding (simply another transformation) to the data table $D$. $V$ is then rendered and rasterized.   Second, it proposes to also model a user task as a function $q(D)$ over the input data table $D$ that the user attempts to estimate using the rendered visual abstraction.   

This separation makes it possible to analyze the relationship between different visualization designs by comparing their design-specific transformations and encodings separately.   
It also helps inform experiment design: rather than measure user responses under varying visual mappings, which confounds the impact of design-specific transformations and visual encodings, experiments can vary each in isolation for proper attribution.
Further, it models both visualization and tasks as functions over the data tables, and thus provides a way to relate the two concepts.  

The rest of this paper first introduces the transform-centric model, and then presents implications to visualization theory and evaluation.



==> content/limitations.tex <==
\section{Limitations}

No perception, cognition in model.

Distinguishing task completion time and accuracy.

Simplified tasks, simplified data model.

